Integrating curation into scientific publishing to train AI models

High throughput extraction and structured labeling of data from academic articles is critical to enable downstream machine learning applications and secondary analyses. We have embedded multimodal data curation into the academic publishing process to annotate segmented figure panels and captions. Natural language processing (NLP) was combined with human-in-the-loop feedback from the original authors to increase annotation accuracy. Annotation included eight classes of bioentities (small molecules, gene products, subcellular components, cell lines, cell types, tissues, organisms, and diseases) plus additional classes delineating the entities' roles in experiment designs and methodologies. The resultant dataset, SourceData-NLP, contains more than 620,000 annotated biomedical entities, curated from 18,689 figures in 3,223 articles in molecular and cell biology. We evaluate the utility of the dataset to train AI models using named-entity recognition, segmentation of figure captions into their constituent panels, and a novel context-dependent semantic task assessing whether an entity is a controlled intervention target or a measurement object. We also illustrate the use of our dataset in performing a multi-modal task for segmenting figures into panel images and their corresponding captions.

==> tables/intro/available_datasets.tex <==

\begin{table}
    \caption{Overview of NER/NEL available datasets.}
    \tiny
    \centering
    \begin{tabularx}{\textwidth}{lcccclllrl}
        \toprule
        \textbf{Dataset} &
        \textbf{NER} &
        \textbf{NEL} &
        \textbf{RE} &
        \textbf{ER} &
        \textbf{Novel} &
        \textbf{Corpora size} &
        \textbf{Entity type} &
        \textbf{\# Mentions} &
        \textbf{References} \\
        \midrule
        BC2GM        & \checkmark     &   &   &   &   & 20,000 sentences           & G                                      & 44,500  & \citealp{bc2gm}                 \\
        BC5DR        & \checkmark     & \checkmark & \checkmark &   &   & 1,500 PubMed Abstracts      & CH, D                                  & 29,271  & \citealp{bc5chem}               \\
        EBM PICO     & \checkmark     &   &   &   &   & 4,993 PubMed Abstracts            & PICO                                   & 71,281  & \citealp{ebm-pico}              \\
        JNLPBA       & \checkmark     &   &   &   &   & 2,404  PubMed Abstracts    & P, DNA, RNA, C line, C type            & 59,963  & \citealp{jnlpba-a}                \\
        NCBI-disease & \checkmark     & \checkmark &   &   &   & 793 PubMed Abstracts        & D                                      & 6,892   & \citealp{ncbidisease}          \\
        AnatEM       & \checkmark     & \checkmark &   &   &   & 1,212 documents            & 12+ entities                           & 13,701  & \citealp{pyysalo2014anatomical} \\
        BC4CHEMD     & \checkmark     &   &   &   &   & 10,000 PubMed Abstracts    & CH                                     & 84,355  & \citealp{KrallingerCHEMDNER}    \\
        BioNLP09     & \checkmark     & \checkmark &   &   &   & 1,210 Abstracts            & P, P regions, C locations              & 15,497  & \citealp{kim-etal-2009-overview} \\
        BioNLP11ID   & \checkmark     & \checkmark & \checkmark &   &   &  316 Abstracts              & P, O, CH, two-component system         &  12,788 &  \citealp{pyysalo-etal-2011-overview} \\
        BioNLP13CG   & \checkmark     & \checkmark & \checkmark &   &   &  600 Abstracts              & 20+ entities                           &  21,654 &  \citealp{pyysalo-etal-2013-overview} \\
        BioNLP13GE   & \checkmark     & \checkmark & \checkmark &   &   & 776 Abstracts               & P, anaphora, binding, entity           & 12,726  & \citealp{kim-etal-2013-genia}   \\
        BioNLP13PC   & \checkmark     & \checkmark & \checkmark &   &   &  525 Abstracts              &  CH, G or GP,  complex, SC             &  15,901 &  \citealp{ohta-etal-2013-overview} \\
        NLM-Gene     & \checkmark     & \checkmark &   &   &   & 550 PMC Articles    & G                                      & 15,411  & \citealp{islamaj2021nlm}        \\
        LINNAEUS     & \checkmark     &   &   &   &   & 100 PMC Articles            & O                                      & 4,259   & \citealp{linnaeus}              \\
        BioRED       & \checkmark     & \checkmark & \checkmark &   & \checkmark & 600 PMC Articles            & G, D, CH, variant, O, C line           & 20,419  & \citealp{biored}                \\
        GENETAG      & \checkmark     &   &   &   &   & 15,000 Sentences           & G                                      & 17,866  & \citealp{genetag}               \\
        GNormPlus    & \checkmark     & \checkmark &   &   &   & 694 PubMed Abstracts               & G, G Family and P Domain               & 10,638   & \citealp{genenormplus}             \\
        MedMentions  & \checkmark     & \checkmark &   &   &   & 4,392 PubMed Abstracts & More than 20 different entities        & 352,312 & \citealp{medmentions}           \\
        \midrule
        SourceData-NLP   & \checkmark & \checkmark &   & \checkmark &   & 18,689 figure captions of 3,223 papers                            & GP, CH, C, T, SC,  O, EA,  D           & 623,162 &  This work                     \\
        \bottomrule
    \end{tabularx}
    \par
    \parbox[]{\textwidth}{
        \tiny{
            \textbf{ER: }Experimental roles, \textbf{GP: }Gene products, \textbf{G: }Genes, \textbf{P: }Proteins, \textbf{C: }Cells,
            \textbf{T: }Tissue, \textbf{SC: }Subcellular, \textbf{O: } Organism or species, \textbf{EA: }Experimental assay,
            \textbf{D: }Disease, \textbf{CH: }Chemicals or small molecules, \textbf{PICO: }Participants, interventions, outcomes
        }
    \label{tab:dataset-overview}
    }
\end{table}


==> tables/methods/journals.tex <==
\begin{table}[!t]
    \label{tab:journals}
    \caption{Distribution of annotated articles per journal.}
    \centering
    \begin{tabularx}{0.5\textwidth}{r|l}
        \toprule 
        \textbf{Journal}                    & \textbf{\# articles}\\
        \midrule
        \textbf{The EMBO Journal}           & 1193\\
        \textbf{EMBO Reports}               & 935 \\
        \textbf{EMBO Molecular Medicine}    & 594 \\
        \textbf{Molecular Systems Biology}  & 169 \\
        \textbf{Nature Cell Biology }       & 51 \\
        \textbf{Nature}                     & 43 \\
        \textbf{The Journal of Cell Biology}& 40 \\
        \textbf{Nature Communications}      & 40 \\
        \textbf{BioRXiv}                    & 38\\
        \textbf{PLOS Pathogens}             & 28 \\
        \textbf{Others}                     & 102\\
        \bottomrule
    \end{tabularx}
    \par
    \parbox[]{0.5\textwidth}{
        \footnotesize{If less than 20 articles have been annotated, the journal is included in "others".}
    }
\end{table}

==> tables/methods/model_property_comparison.tex <==
\begin{table}
    \caption{Comparison of the high-level properties of the benchmark models.}
    \label{tab:models}
    \centering
    \begin{tabularx}{\textwidth}{l|cclll}
        \toprule
        \textbf{Model}        & \textbf{Param.} & \textbf{Corpora}      & \textbf{Tokenization} & \textbf{Pretraining} & \textbf{Ref.}\\
        \midrule
        BioLinkBERT$_{base}$  & 108M            & BERT + PubMed$_{abs}$ & WP-bio                & PubMedBERT           & \cite{biolinkbert}\\
        BioLinkBERT$_{large}$ & 333M            & BERT + PubMed$_{abs}$ & WP-bio                & PubMedBERT           & \cite{biolinkbert}\\
        PubMedBERT            & 109M            & PubMed                & WP-bio                & -                    & \cite{pubmedbert}\\
        PubMedBERT            & 333M            & PubMed                & WP-bio                 & -                   & \cite{pubmedbert}\\
        \bottomrule
    \end{tabularx}
\end{table}

==> tables/results/entity_linking.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|c|c|c}
\toprule
         \textbf{Entity Type} & \textbf{@1} & \textbf{@5} & \textbf{@10} \\
         % & & & \\
\midrule
         \textbf{Gene Products} & & & \\
         \tab - species prediction & & & \\ 
        \textbf{Cell Line}	   & 0.9194	& 0.9749	& 0.9755\\
        \textbf{Cell Type}	   & 0.6761	& 0.8021	& 0.8344 \\
        \textbf{Disease}	       & 0.5198	& 0.6446	& 0.6484 \\
        \textbf{Exp. Assay}	   & 0	    & 0	        & 0 \\
        \textbf{Subcellular}	   & 0.7096	& 0.8274	& 0.8524 \\
        \textbf{Tissue}	       & 0.0131	& 0.0131	& 0.0131 \\
        \textbf{Small Mol.} &0.4807	& 0.6587	& 0.6727 \\

\bottomrule
    \end{tabular}
    \caption{Named entity linking results for each entity type}
    \label{tab:entity_linking}
\end{table}

==> tables/results/ner_f1_scores.tex <==
\begin{table}
    \centering
    \caption{F1 scores of single- and multi-class models for each entity category.}
    \label{tab:multi-vs-single}
    \begin{tabularx}{0.7\textwidth}{lrrc|rc}
        \toprule
        Class          & Single         & Multi$_{avg}$ & $\Delta_{avg}\% $ & Multi$_{best}$ & $\Delta_{best}\%$\\
        \midrule
        Gene product   & 91.8           & 91.5          & -0.3     &  \textbf{92.7}  & 1.0\\
        Cell line      & \textbf{91.3}  & 90.4          & -1.0     &  90.8           & -0.6\\
        Organism       & 87.4           & 87.4          & 0.0      &  \textbf{87.8}  & 0.5\\
        Small Molecule & 85.0           & 84.7          & -0.3     &  \textbf{86.2}  & 1.4\\
        Tissue         & \textbf{83.5}  & 83.1          & -0.4     &  \textbf{83.5}  & 0.0\\
        Subcellular    & 78.7           & 79.3          & 0.8      &  \textbf{79.6}  & 1.1\\
        Cell type      & 72.4           & 72.1          & -0.4     &  \textbf{72.6}  & 0.3\\
        Disease        & 67.4           & 67.7          & 0.4      &  \textbf{69.5}  & 3.0\\
        Exp. Assay     & 68.2           & 67.7          & -0.7     &  \textbf{68.7}  & 0.7\\
        \midrule
        Macro average  & 80.6           & 80.5          & 12.4     &  \textbf{81.3}  & 0.8\\
        \bottomrule
    \end{tabularx}
    \par
    \parbox[]{0.7\textwidth}{
        \footnotesize{
             The percentage difference between both ($\Delta_{avg}\%$ for the mean multi-model and $\Delta_{best}\% $ for the best multi-model) is estimated as $\left (1 - \frac{S}{M} \right )$. The best scores are highlighted in bold. The multi-class F1 scores are obtained as the macro-averages of the four models trained in Section~\ref{sec:multi-class}.
        }
    }
\end{table}


==> tables/results/roles-gp.tex <==
\begin{table}[h!!]
    \caption{Micro averaged F1 scores of the empirical role of entities task for gene products for the context only, marked-entity, and single-step approaches.}
    \label{tab:results-roles}
    \begin{tabularx}{\textwidth}{clllll}
        \toprule
                                   & \multicolumn{5}{c}{Micro averaged F1}                                                 \\
        \cline{2-6} 
        \textbf{Model}             & Context-only & Context only corr. & Marked-entity & Marked-entity corr. & Single-step \\
        \midrule
        \textbf{PubMedBERT-base}   & 91.2         & 83.8               & 91.6          & 84.2                & 81.4        \\
        \textbf{PubMedBERT-large}  & 91.0         & 84.0               & 92.3          & 85.2                & 82.5        \\
        \bottomrule
    \end{tabularx}
    % \par
    % \parbox[]{\textwidth}{
    %     \footnotesize{For the approaches that need NER on inference (context only and marked-entity), we also provide the corrected F1 score by multiplying the F1 scores of the role classification step by the respective NER score in Table~\ref{tab:ner}.}
    % }
\end{table}

